Local existence of smooth solutions for the semigeostrophic equations on curved domains

We prove local-in-time existence of smooth solutions to the semigeostrophic equations in the general setting of smooth, bounded and simply connected domains of $\mathbb{R}^2$ endowed with an arbitrary conformally flat metric and non-vanishing Coriolis term. We present a construction taking place in Eulerian coordinates, avoiding the classical reformulation in dual variables, used in the flat case with constant Coriolis force, but lacking in this general framework.

==> appendices.tex <==
\section{Sobolev embeddings and interpolation}\label{appendix:Sobolev_interpolation}
\begin{theorem}[Adams interpolation]\label{thm:Adams}Let $\Om\subset\R^n$ be any bounded and smooth domain. Then, for every $0\leq k\leq m$ there exists a constant $c=c(k,m,\Om)>0$ such that
\[
\norm{v}_{H^k(\Om)}\leq c\norm{v}_{L^2(\Om)}^{1-\frac{k}{m}}\norm{v}_{H^m(\Om)}^{\frac{k}{m}},
\]
for every $v\in H^m(\Om)$.
\end{theorem}
\begin{proof}
The detailed proof can be found in \cite[Chapter 5]{A08}. As a side remark, notice that the authors proved this result only assuming $\Om$ satisfying some suitable "weak cone condition".
\end{proof}
The following proposition is a small variation of Lemma 3.4  in \cite{MB01} (for our purposes, we specialize it from $\R^2$ to $\Om$. The proof is essentially the same).
\begin{proposition}[Interpolation inequalities]Let $\Om\subset \R^2$ be any smooth and bounded domain, and  let $v,w$ be functions in $H^r(\Om)$. Then, there exists $C=C(r,\Om)>0$ such that
\begin{equation}\label{eq:banach_algebra}
\norm{D^\alpha(vw)}_{L^2(\Om)}\leq C\Bigl(\norm{v}_{L^\infty(\Om)}\norm{w}_{H^r(\Om)}+\norm{w}_{L^\infty(\Om)}\norm{v}_{H^r(\Om)}\Bigr),
\end{equation}
for all multi-index $\abs{\alpha}=r$.
In particular, the following inequalities
\begin{equation}\label{eq:interpol_1}
\norm{D^\alpha (vw)-vD^\alpha w}_{L^2(\Om)}\leq C_r\Bigl(\norm{\nabla v}_{L^\infty(\Om)}\norm{w}_{H^{r-1}(\Om)}+\norm{v}_{H^r(\Om)}\norm{w}_{L^\infty(\Om)}\Bigr),
\end{equation}
and
\begin{equation}\label{eq:interpol_2}
\norm{D^\alpha(vw)-vD^\alpha w-wD^\alpha v}_{L^2(\Om)}\leq C_r\Bigl(\norm{\nabla v}_{L^\infty(\Om)}\norm{w}_{H^{r-1}(\Om)}+\norm{v}_{H^{r-1}(\Om)}\norm{\nabla w}_{L^\infty(\Om)}\Bigr),
\end{equation}
hold.
\end{proposition}
\begin{proof}
First of all, recall the following particular case of the Gagliardo-Nirenberg inequality: for every $r\geq 0$ there exists $C_r>0$ such that for every $i\leq r$ the following estimate
\begin{equation}\label{eq:GN}
\norm{D^i h}_{L^{2r/i}(\Om)}\leq C_r\norm{h}^{1-i/r}_{L^\infty(\Om)}\norm{D^r h}_{L^2(\Om)}^{i/r}+C_{r,\Om}\norm{h}_{L^2(\Om)},
\end{equation}
hold. Here, the last term compensate the fact that we consider a bounded and smooth domain $\Om$ instead of the whole plane $\R^2$  (see \cite[Page 126]{N60}).
Now, let $\abs{\alpha}=r$. By the Leibnitz rule and Hölder inequality we have that there exists $C_\alpha>0$ such that
\begin{align*}
\norm{D^\alpha(vw)}_{L^2(\Om)}\leq C_\alpha\sum_{\gamma+\beta=\alpha}\norm{D^\gamma vD^\beta w}_{L^2(\Om)}\leq C_\alpha\sum_{\gamma+\beta=\alpha}\norm{D^\gamma v}_{L^{\frac{2r}{\abs{\gamma}}}(\Om)}\norm{D^\beta w}_{L^{\frac{2r}{\abs{\beta}}}(\Om)},
\end{align*}
which, by \eqref{eq:GN}, we can estimate as
\begin{align*}
\norm{D^\alpha(vw)}_{L^2(\Om)}&\leq C_{\alpha,\Om}\sum_{\gamma+\beta=\alpha}\Bigl(\norm{v}_{L^\infty(\Om)}^{1-\frac{\abs{\gamma}}{r}}\norm{D^r v}_{L^2(\Om)}^{\frac{\abs{\gamma}}{r}}+\norm{v}_{L^2(\Om)}\Bigr)\Bigl(\norm{w}_{L^\infty(\Om)}^{1-\frac{\abs{\beta}}{r}}\norm{D^ r w}_{L^2(\Om)}^{\frac{\abs{\beta}}{r}}+\norm{w}_{L^2(\Om)}\Bigr)\\
&\leq C'_{\alpha,\Om}\sum_{i=0}^r\Biggl(\Bigl(\norm{v}_{L^\infty(\Om)}\norm{D^r w}_{L^2(\Om)}\Bigr)^{1-\frac{i}{r}}\Bigl(\norm{w}_{L^\infty(\Om)}\norm{D^r v}_{L^2(\Om)}\Bigr)^{\frac{i}{r}}\\
&\quad+\norm{w}_{L^2(\Om)}\norm{v}_{L^\infty(\Om)}^{1-\frac{i}{r}}\norm{D^r v}_{L^2(\Om)}^{\frac{i}{r}}+\norm{v}_{L^2(\Om)}\norm{w}_{L^\infty(\Om)}^{1-\frac{i}{r}}\norm{D^r w}_{L^2(\Om)}^{\frac{i}{r}}\Biggr)\\
&\leq C'_{\alpha,\Om}\Biggl(\Bigl(\norm{v}_{L^\infty(\Om)}\norm{D^r w}_{L^2(\Om)}+\norm{w}_{L^\infty(\Om)}\norm{D^r v}_{L^2(\Om)}\Bigr)\\
&\quad+\norm{w}_{L^2(\Om)}\Bigl(\norm{v}_{L^\infty(\Om)}+\norm{D^r v}_{L^2(\Om)}\Bigr)+\norm{v}_{L^2(\Om)}\Bigl(\norm{w}_{L^\infty(\Om)}+\norm{D^r w}_{L^2(\Om)}\Bigr)\Biggr).
\end{align*}
Since $\Om$ is bounded, then $L^\infty(\Om)\subset L^2(\Om)$, and therefore
\[
\norm{D^\alpha(vw)}_{L^2(\Om)}\leq C''_{\alpha,\Om}\Bigl(\norm{v}_{L^\infty(\Om)}\norm{w}_{H^r(\Om)}+\norm{w}_{L^\infty(\Om)}\norm{v}_{H^r(\Om)}\Bigr),
\]
for some $C''_{\alpha,\Om}>0$, proving \eqref{eq:banach_algebra}. Estimates \eqref{eq:interpol_1} and \eqref{eq:interpol_2} can be obtained in the exact same fashion simply observing that
\[
\norm{D^{\alpha}(vw)-vD^\alpha w}_{L^2(\Om)}\leq C_\alpha\sum_{\abs{\gamma}+\abs{\beta}\leq r-1}\norm{D^\gamma(\nabla v)D^\beta w}_{L^2(\Om)},
\] 
and
\[
\norm{D^{\alpha}(vw)-vD^\alpha w-wD^\alpha v}_{L^2(\Om)}\leq C_\alpha\sum_{\abs{\gamma}+\abs{\beta}\leq r-2}\norm{D^\gamma(\nabla v)D^\beta (\nabla w)}_{L^2(\Om)}.
\] 
\end{proof}
\begin{remark}In particular, if $r\geq 2$, Equation \eqref{eq:banach_algebra} implies that $H^r(\Om)$ is a Banach algebra, and if $\abs{\alpha}=r\geq 4$, then by the Sobolev embeddings $H^{2+s}(\Om)\hookrightarrow W^{s,\infty}(\Om)$ we have that
\begin{equation*}
\norm{D^\alpha (vw)-vD^\alpha w}_{L^2(\Om)}\leq C_r\norm{v}_{H^r(\Om)}\norm{w}_{H^{r-1}(\Om)},
\end{equation*}
and
\begin{equation*}
\norm{D^\alpha(vw)-vD^\alpha w-wD^\alpha v}_{L^2(\Om)}\leq C_r\norm{v}_{H^{r-1}(\Om)}\norm{w}_{H^{r-1}(\Om)}.
\end{equation*}
\end{remark}

==> derivation.tex <==
In this section we briefly describe the derivation of the semigeostrophic equation starting from the classical Euler equation governing the evolution of an inviscid fluid on the surface of  a rotating sphere. The generalization to conformally flat domains follows naturally after projecting everything stereographically. Consider the two dimensional sphere  $\mathbb{S}^2$ rotating on itself with constant velocity $\omega$. The canonical Riemannian metric is given in spherical coordinates $(\theta,\phi)$ by
\[
g=d\theta^2+\sin(\theta)d\phi^2,
\]
where $\theta\in(0,\pi)$ represents the latitude and $\phi\in (0,2\pi)$ the longitude. Denoting with $D^g$, $\diva^g$ and  $\nabla_g$ the Levi-Civita connection, the divergence and the gradient operator  associated  to $g$, and with $(\cdot)^\perp$ the counter-clockwise rotation of $\pi/2$ radians, the  evolution of a two dimensional inviscid fluid on this sphere is described by
\begin{equation}\label{eq:Euler}
\begin{cases}
(\partial_t+D^g_u)u+fu^\perp+\nabla_g p=0,\\
\diva^g(u)=0,
\end{cases}
\end{equation}
where $u$  and $p$ represent respectively the velocity and the pressure of the fluid, and $f$ is the Coriolis term which equal to $f=2\omega\cos(\theta)$. In the large scale setting it is believed that force induced by the rotation dominates the advection term (at least far form the equator). This induce the definition of a new quantity $u_G$, called the geostrophic wind, which represents the balance
\[
fu_G^\perp+\nabla_g p=0.
\]
Equivalently, we can simply  set $u_G:=\frac{1}{f}\nabla_g^\perp p$. The semigeostrophic approximation consists into neglecting the action of the material derivative on the difference $u-u_G$ (called the  ageostrophic component of the wind), but preserving all information about the fluid velocity in the remaining terms of the equation. This means that we are asking
\[
\partial_t u_G+D^g_u u_G+fu^\perp+\nabla_g p=0.
\]
In a more compact form, we finally have the semigeostrophic equation
\begin{equation}\label{eq:primitive_SG}
\begin{cases}
(\partial_t+D^g_u)u_G+f(u-u_G)^\perp=0,\\
u_G=\frac{1}{f}\nabla^\perp_g p,\\
\diva^g(u)=0,\\
\end{cases}
\end{equation}
in its essential formulation (see \cite[Chapter 2]{C06} for the spherical case, and  \cite[Chapter 1]{C06}, \cite{H75} and \cite{L06} for the flat periodic one). Operating a stereographic projection pointed  at the South Pole,  we can see \eqref{eq:primitive_SG} as taking place in the two dimensional plane endowed with the conformal metric and Coriolis term
\begin{equation}\label{eq:spherical_coeff}
g=\frac{4}{(1+\abs{x}^2)^2}\bigl((dx^1)^2+(dx^2)^2\bigr),\,f=2\omega\frac{1-\abs{x}^2}{1+\abs{x}^2},
\end{equation}
in canonical Cartesian coordinates $(x^1,x^2)$. We  decided to solve the semigeostrophic equation in a smooth, bounded and simply connected domain $\Om$ of the stereographic plane, prescribing the velocity vector field $u$ tangent to $\partial\Om$, which corresponds to the natural condition for mass preservation. We also ask $\Om$ to be sufficiently far form the equator $\partial B(0,1)$ since there $f^{-1}$ diverges badly.\\
\par To summarise, we can give the general statement of this problem: let $\Om$ be a sufficiently smooth, bounded and simply connected domain of $\R^2$, and let $V,\varphi$ be two given smooth functions defined on $\bar\Om$. Set $g:=e^{-2V}\bigl((dx^1)^2+(dx^2)^2\bigr)$ and $f=e^{-\varphi}$, and define the endomorphism of tangent bundle
\[
J=(\cdot)^\perp:T\Om\to T\Om,\, J=-dx^2\otimes\frac{\partial}{\partial x^1}+dx^1\otimes\frac{\partial}{\partial x^2},
\]
to be the counter-clockwise rotation of $\pi/2$-radians. Given an initial pressure gradient $\nabla^g p_0$ satisfying some suitable assumptions, we ask ourselves if it is possible to find a local-in-time smooth solution of the  semigeostrophic system
\begin{equation}\label{eq:SG}
\begin{cases}
(\partial_t+D^g_u)\bigl(e^{\varphi}\nabla_g^\perp p\bigr)+e^{-\varphi}\bigl(u-e^{\varphi}\nabla^\perp_g p\bigr)^\perp=0,&\text{ in }\Om,\\
\diva^g(u)=0,&\text{ in }\Om,\\
g(u,\nu)=0,&\text{ on }\partial\Om,\\
\nabla^gp_t\mid_{t=0}=\nabla^gp_0,
\end{cases}
\end{equation}
where $\nu$ denotes the outer pointing normal vector to $\partial\Om$. In particular, when $\varphi$ and $V$ are as in \eqref{eq:spherical_coeff}  we are in the spherical case, and when $V=\varphi=0$, we are in the classical flat case. As a side remark, we will see at the end that our method works also in the non-simply connected periodic situation $\Om=\T^2$.
